Context-aware Fine-tuning of Self-supervised Speech Models

Self-supervised pre-trained transformers have improved the state of the art on a variety of speech tasks. Due to the quadratic time and space complexity of self-attention, they usually operate at the level of relatively short (e.g., utterance) segments. In this paper, we study the use of context, i.e., surrounding segments, during fine-tuning and propose a new approach called context-aware fine-tuning. We attach a context module on top of the last layer of a pre-trained model to encode the whole segment into a context embedding vector which is then used as an additional feature for the final prediction. During the fine-tuning stage, we introduce an auxiliary loss that encourages this context embedding vector to be similar to context vectors of surrounding segments. This allows the model to make predictions without access to these surrounding segments at inference time and requires only a tiny overhead compared to standard fine-tuned models. We evaluate the proposed approach using the SLUE and Libri-light benchmarks for several downstream tasks: Automatic speech recognition (ASR), named entity recognition (NER), and sentiment analysis (SA). The results show that context-aware fine-tuning not only outperforms a standard fine-tuning baseline but also rivals a strong context injection baseline that uses neighboring speech segments during inference.

==> sections/related_work.tex <==
\section{Related work}
\label{sec:related}

In NLP, relationing between utterances in training objective was explored on learning large language model. BERT~\cite{devlin2018bert} has next sentence prediction, abandoned by RoBerta~\cite{liu2019roberta} while Albert~\cite{lan2019albert} found sentence order prediction worth
\felix{Skip-Thought Vectors\cite{kiros2015skip} might be the first paper in NLP to do it.}


In speech, similar relationing was done in such as APC~\cite{chung2019unsupervised}, CPC~\cite{oord2018representation}, MPC~\cite{baevski2020wav2vec}. However, this was done in audio frame-level that is very short-term context less than 100msec.

Recent study~\cite{an2022cuside,kim2021multi} tried to simulating or encoding future context, but still in very short-term future.

This work~\cite{kim2019acoustic,kim2019cross} tried to use previous text token or previous conversational dialog texts as for context conditioning. \cite{kim2019acoustic} need separated training for context embedding. \cite{kim2019cross}, although it can be trained end-to-end, two channel need to be process synchronously. Most of all, two approach need previous decoded text in inference time.

Related papers \cite{narayanan2019recognizing,hori2021advanced}



==> tables/table_asr.tex <==

\begin{table}[!htp]\centering
\caption{WER on SLUE-Voxceleb ASR task}\label{tab:asr_voxceleb}
% \scriptsize
\begin{tabular}{lrrrrr}\toprule
\multirow{2}{*}{\makecell{Fine-tuning\\model}} &\multicolumn{2}{c}{dev} &\multicolumn{2}{c}{test} \\\cmidrule{2-5}
&without LM &with LM &without LM &with LM \\\midrule
(a) &17.5 &13.3 &20.9 &16.1 \\
(b) &16.7 &12.7 &20.1 &15.8 \\
(c) &16.7 &12.8 &20.0 &15.8 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!htp]\centering
\caption{WER on SLUE-Voxpopuli ASR task}\label{tab:asr_voxpopuli}
% \scriptsize
\begin{tabular}{lrrrrr}\toprule
\multirow{2}{*}{\makecell{Fine-tuning\\model}} &\multicolumn{2}{c}{dev} &\multicolumn{2}{c}{test} \\\cmidrule(l{2pt}r{2pt}){2-3} \cmidrule(l{2pt}r{2pt}){4-5}
&without LM &with LM &without LM &with LM \\\midrule
(a)\cite{shon2022slue} &17.5 &12.0 &18.4 &12.3 \\
(b) &16.6 &12.0 &17.4 &12.2 \\
(c) &16.4 &11.8 &17.0 &12.1 \\
\bottomrule
\end{tabular}
\end{table}




==> tables/table_ner.tex <==
\begin{table}[!tp]\centering
\caption{F1 score on SLUE-Voxpopuli NER task.}\label{tab:ner}
% \scriptsize
\begin{tabular}{lrrrrr}\toprule
\multirow{2}{*}{\makecell{Fine-tuning\\model}} &\multicolumn{2}{c}{dev} &\multicolumn{2}{c}{test} \\\cmidrule{2-5}
&without LM &with LM &without LM &with LM \\\midrule
(a)\cite{shon2022slue} &55.0 &68.1 &49.6 &63.4 \\
(b) &60.0 &69.8 &53.8 &64.0 \\
(c) &60.1 &70.1 &55.0 &64.1 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/table_sent.tex <==
\begin{table}[!tp]\centering
\caption{F1 score on SLUE-Voxceleb sentiment analysis. *:We found the baseline in~\cite{shon2022slue} is fairly low performing compared to our reproduced baseline model. Thus we reported an updated numbers on baseline model}\label{tab:sentiment}
% \scriptsize
\begin{tabular}{lrrr}\toprule
\makecell{Fine-tuning\\model} &dev &test \\\midrule
(a)\cite{shon2022slue} &43.3 &48.6 \\
(a)* &49.2 &51.8 \\
(b) &49.8 &52.1 \\
(c) &49.7 &52.9 \\
\bottomrule
\end{tabular}
\end{table}
